Demand for LLMs: Descriptive Evidence on Substitution, Market Expansion, and Multihoming

This paper documents three stylized facts about the demand for Large Language Models (LLMs) using data from OpenRouter, a prominent LLM marketplace. First, new models experience rapid initial adoption that stabilizes within weeks. Second, model releases differ substantially in whether they primarily attract new users or substitute demand from competing models. Third, multihoming, using multiple models simultaneously, is common among apps. These findings suggest significant horizontal and vertical differentiation in the LLM market, implying opportunities for providers to maintain demand and pricing power despite rapid technological advances.

==> tables/price_elasticity.tex <==

\begingroup
\centering
\begin{tabular}{lc}
   \toprule
   Dependent Variable:     & Log Tokens\\  
   Model:                  & (1)\\  
   \midrule
   \emph{Variables}\\
   Log Output Price        & -0.308$^{***}$\\   
                           & (0.107)\\   
   Log Context Window Size & 0.659$^{***}$\\   
                           & (0.165)\\   
   \midrule
   \emph{Fixed-effects}\\
   date                    & Yes\\  
   provider                & Yes\\  
   \midrule
   \emph{Fit statistics}\\
   Observations            & 13,970\\  
   R$^2$                   & 0.40236\\  
   \bottomrule
   \multicolumn{2}{l}{\emph{Clustered (model) standard-errors in parentheses}}\\
   \multicolumn{2}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\
\end{tabular}
\par\endgroup




==> tables/top_10_apps.tex <==
\begin{table}[!h]
\centering
\caption{Top 10 Applications by Token Usage}
\centering
\begin{tabular}[t]{ll}
\toprule
Application & Usage (Millions of Tokens)\\
\midrule
\cellcolor{gray!10}{Cline} & \cellcolor{gray!10}{314 583 M}\\
Roo Code & 231 702 M\\
\cellcolor{gray!10}{shapes inc} & \cellcolor{gray!10}{37 620 M}\\
SillyTavern & 36 883 M\\
\cellcolor{gray!10}{Chub AI} & \cellcolor{gray!10}{17 435 M}\\
\addlinespace
DocsLoop & 14 264 M\\
\cellcolor{gray!10}{OpenRouter: Chatroom} & \cellcolor{gray!10}{13 405 M}\\
liteLLM & 11 461 M\\
\cellcolor{gray!10}{Fraction AI} & \cellcolor{gray!10}{8 085 M}\\
Fish Audio & 6 445 M\\
\bottomrule
\end{tabular}
\end{table}
